Deep Learning-Based Anomaly Detection in Cyber-Physical Systems: Progress and Opportunities

Anomaly detection is crucial to ensure the security of cyber-physical systems (CPS). However, due to the increasing complexity of CPSs and more sophisticated attacks, conventional anomaly detection methods, which face the growing volume of data and need domain-specific knowledge, cannot be directly applied to address these challenges. To this end, deep learning-based anomaly detection (DLAD) methods have been proposed. In this paper, we review state-of-the-art DLAD methods in CPSs. We propose a taxonomy in terms of the type of anomalies, strategies, implementation, and evaluation metrics to understand the essential properties of current methods. Further, we utilize this taxonomy to identify and highlight new characteristics and designs in each CPS domain. Also, we discuss the limitations and open problems of these methods. Moreover, to give users insights into choosing proper DLAD methods in practice, we experimentally explore the characteristics of typical neural models, the workflow of DLAD methods, and the running performance of DL models. Finally, we discuss the deficiencies of DL approaches, our findings, and possible directions to improve DLAD methods and motivate future research.

==> sections/acmpapertable.tex <==
ACM DL for AD in CPS:

\begin{itemize}
    \item Schneider, Peter, and Konstantin Böttinger. "High-Performance Unsupervised Anomaly Detection for Cyber-Physical System Networks." In Proceedings of the 2018 Workshop on Cyber-Physical Systems Security and PrivaCy, pp. 1-12. ACM, 2018.   7  c
    \item Khanapuri, Eshaan, Tarun Chintalapati, Rajnikant Sharma, and Ryan Gerdes. "Learning-based adversarial agent detection and identification in cyber physical systems applied to autonomous vehicular platoon." In 2019 IEEE/ACM 5th International Workshop on Software Engineering for Smart Cyber-Physical Systems (SEsCPS), pp. 39-45. IEEE, 2019.  0  c
    % \item Lane, Nicholas D., Sourav Bhattacharya, Petko Georgiev, Claudio Forlivesi, and Fahim Kawsar. "An early resource characterization of deep learning on wearables, smartphones and internet-of-things devices." In Proceedings of the 2015 international workshop on internet of things towards applications, pp. 7-12. ACM, 2015.  107  measure performance at resource-constrained devices
    % \item Cho, Sungjin, Fumin Zhang, and Catherine Edwards. "Detecting Abnormal Speed of Marine Robots using Controlled Lagrangian Particle Tracking Methods." In Proceedings of the International Conference on Underwater Networks \& Systems, p. 11. ACM, 2017.  0 control theory ML
    \item Hundman, Kyle, Valentino Constantinou, Christopher Laporte, Ian Colwell, and Tom Soderstrom. "Detecting spacecraft anomalies using lstms and nonparametric dynamic thresholding." In Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovelocityvery \& Data Mining, pp. 387-395. ACM, 2018.   28   c
    \item Kravchik, Moshe, and Asaf Shabtai. "Detecting cyber attacks in industrial control systems using convolutional neural networks." In Proceedings of the 2018 Workshop on Cyber-Physical Systems Security and PrivaCy, pp. 72-83. ACM, 2018.       16    c
    \item Zohrevand, Zahra, Uwe Glässer, Mohammad A. Tayebi, Hamed Yaghoubi Shahir, Mehdi Shirmaleki, and Amir Yaghoubi Shahir. "Deep learning based forecasting of critical infrastructure data." In Proceedings of the 2017 ACM on Conference on Information and Knowledge Management, pp. 1129-1138. ACM, 2017.       5   c
    \item Su, Ya, Youjian Zhao, Chenhao Niu, Rong Liu, Wei Sun, and Dan Pei. "Robust Anomaly Detection for Multivariate Time Series through Stochastic Recurrent Neural Network." In Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining, pp. 2828-2837. ACM, 2019.     0  c
    \item Tariq, Shahroz, Sangyup Lee, Youjin Shin, Myeong Shin Lee, Okchul Jung, Daewon Chung, and Simon S. Woo. "Detecting Anomalies in Space using Multivariate Convolutional LSTM with Mixtures of Probabilistic PCA." In Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining, pp. 2123-2133. ACM, 2019.     0  c
\end{itemize}

IEEE DL for AD in CPS:

\begin{itemize}
    \item Tasfi, Norman L., Wilson A. Higashino, Katarina Grolinger, and Miriam AM Capretz. "Deep neural networks with confidence sampling for electrical anomaly detection." In 2017 IEEE International Conference on Internet of Things (iThings) and IEEE Green Computing and Communications (GreenCom) and IEEE Cyber, Physical and Social Computing (CPSCom) and IEEE Smart Data (SmartData), pp. 1038-1045. IEEE, 2017.           5   c
    \item Ezeme, Okwudili M., Qusay H. Mahmoud, and Akramul Azim. "Dream: deep recursive attentive model for anomaly detection in kernel events." IEEE Access 7 (2019): 18860-18870.        1 c
    \item Dimensionality Reduction and Anomaly Detection for CPPS Data using Autoencoder          0   c
    % \item Pandey, Ankur, Ryan Sequeria, Preetam Kumar, and Sudhir Kumar. "A Multistage Deep Residual Network for Biomedical Cyber-Physical Systems." IEEE Systems Journal (2019).        0  not cps
    \item Zhang, Y., V. V. G. Krishnan, J. Pi, K. Kaur, A. Srivastava, A. Hahn, and S. Suresh. "Cyber physical security analytics for transactive energy systems." IEEE Transactions on Smart Grid (2019).      0 c
    \item Liu, Chao, Kin Gwn Lore, and Soumik Sarkar. "Data-driven root-cause analysis for distributed system anomalies." In 2017 IEEE 56th Annual Conference on Decision and Control (CDC), pp. 5745-5750. IEEE, 2017.  3 c
    \item Wang, Jingyu, Dongyuan Shi, Yinhong Li, Jinfu Chen, Hongfa Ding, and Xianzhong Duan. "Distributed framework for detectivelocityng PMU data manipulation attacks with deep autoencoders." IEEE Transactions on Smart Grid (2018).  2 c
    \item Real-Time Sensor Anomaly Detection and Identification in Automated Vehicles       0 c
    % \item Liao, Weixian, Yifan Guo, Xuhui Chen, and Pan Li. "A Unified Unsupervised Gaussian Mixture Variational Autoencoder for High Dimensional Outlier Detection." In 2018 IEEE International Conference on Big Data (Big Data), pp. 1208-1217. IEEE, 2018.       1 not cps
    % \item Zhang, Xiaodong, Matthew Clark, Kudip Rattan, Jonathan Muse, and Mohsen Khalili. "Controller integrity monitoring in adaptive learning systems towards trusted autonomy." IEEE Transactions on Automation Science and Engineering 13, no. 2 (2016): 491-501.     4 too much theory
    % \item Jensen, L., G. Brown, X. Wang, J. Harer, and S. Chin. "Deep Learning for Minimal-context Block Tracking through Side-channel Analysis." In ICASSP 2019-2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), pp. 3207-3211. IEEE, 2019.       0 not anomaly detection
    \item Taylor, Adrian, Sylvain Leblanc, and Nathalie Japkowicz. "Anomaly detection in automobile control network data with long short-term memory networks." In 2016 IEEE International Conference on Data Science and Advanced Analytics (DSAA), pp. 130-139. IEEE, 2016.    81  c
    \item Goh, Jonathan, Sridhar Adepu, Marcus Tan, and Zi Shan Lee. "Anomaly detection in cyber physical systems using recurrent neural networks." In 2017 IEEE 18th International Symposium on High Assurance Systems Engineering (HASE), pp. 140-145. IEEE, 2017.   45 c
    % \item Guo, Tian, Zhao Xu, Xin Yao, Haifeng Chen, Karl Aberer, and Koichi Funaya. "Robust online time series prediction with recurrent neural networks." In 2016 IEEE International Conference on Data Science and Advanced Analytics (DSAA), pp. 816-825. Ieee, 2016.   36 not cps
    \item Feng, Cheng, Tingting Li, and Deeph Chana. "Multi-level anomaly detection in industrial control systems via package signatures and lstm networks." In 2017 47th Annual IEEE/IFIP International Conference on Dependable Systems and Networks (DSN), pp. 261-272. IEEE, 2017.  38 c
    \item Inoue, Jun, Yoriyuki Yamagata, Yuqi Chen, Christopher M. Poskitt, and Jun Sun. "Anomaly detection for a water treatment system using unsupervised machine learning." In 2017 IEEE International Conference on Data Mining Workshops (ICDMW), pp. 1058-1065. IEEE, 2017.     25  c
    \item Deng, Qingyu, and Jian Sun. "False Data Injection Attack Detection in a Power Grid Using RNN." In IECON 2018-44th Annual Conference of the IEEE Industrial Electronics Society, pp. 5983-5988. IEEE, 2018.   0  c
    \item Russo, Michele, Maxime Labonne, Alexis Olivereau, and Mohammad Rmayti. "Anomaly Detection in Vehicle-to-Infrastructure Communications." In 2018 IEEE 87th Vehicular Technology Conference (VTC Spring), pp. 1-6. IEEE, 2018.   0 c
    % \item Shukla, Raj Mani, and Shamik Sengupta. "Analysis and Detection of Outliers due to Data Falsification Attacks in Vehicular Traffic Prediction Application." In 2018 9th IEEE Annual Ubiquitous Computing, Electronics \& Mobile Communication Conference (UEMCON), pp. 688-694. IEEE, 2018.   0  no DNN
    \item Ferrari, P., S. Rinaldi, E. Sisinni, F. Colombo, F. Ghelfi, D. Maffei, and M. Malara. "Performance evaluation of full-cloud and edge-cloud architectures for Industrial IoT anomaly detection based on deep learning." In 2019 II Workshop on Metrology for Industry 4.0 and IoT (MetroInd4. 0\&IoT), pp. 420-425. IEEE, 2019.     0  c
    \item Gunn, Lachlan, Peter Smet, Edward Arbon, and Mark D. McDonnell. "Anomaly Detection in Satellite Communications Systems using LSTM Networks." In 2018 Military Communications and Information Systems Conference (MilCIS), pp. 1-6. IEEE, 2018.        0 c
    \item Kieu, Tung, Bin Yang, and Christian S. Jensen. "Outlier detection for multidimensional time series using deep neural networks." In 2018 19th IEEE International Conference on Mobile Data Management (MDM), pp. 125-134. IEEE, 2018.    13 c
    \item Legrand, Adrien, Brad Niepceron, Alain Cournier, and Harold Trannois. "Study of Autoencoder Neural Networks for Anomaly Detection in Connected Buildings." In 2018 IEEE Global Conference on Internet of Things (GCIoT), pp. 1-5. IEEE, 2018.        0  c
    \item Zhu, Konglin, Zhicheng Chen, Yuyang Peng, and Lin Zhang. "Mobile Edge Assisted Literal Multi-Dimensional Anomaly Detection of In-Vehicle Network Using LSTM." IEEE Transactions on Vehicular Technology 68, no. 5 (2019): 4275-4284.       0 c
    %  \item Zheng, Zibin, Yatao Yang, Xiangdong Niu, Hong-Ning Dai, and Yuren Zhou. "Wide and deep convolutional neural networks for electricity-theft detection to secure smart grids." IEEE Transactions on Industrial Informatics 14, no. 4 (2017): 1606-1615.     29
    \item Niu, Xiangyu, Jiangnan Li, Jinyuan Sun, and Kevin Tomsovic. "Dynamic detection of false data injection attack in smart grid using deep learning." In 2019 IEEE Power \& Energy Society Innovative Smart Grid Technologies Conference (ISGT), pp. 1-6. IEEE, 2019.    1  c
    % \item Liu, Junjiao, Libo Yin, Yan Hu, Shichao Lv, and Limin Sun. "A Novel Intrusion Detection Algorithm for Industrial Control Systems Based on CNN and Process State Transition." In 2018 IEEE 37th International Performance Computing and Communications Conference (IPCCC), pp. 1-8. IEEE, 2018.   0
    % \item Lavrova, Daria, Dmitry Zegzhda, and Anastasiia Yarmak. "Using GRU neural network for cyber-attack detection in automated process control systems." In 2019 IEEE International Black Sea Conference on Communications and Networking (BlackSeaCom), pp. 1-3. IEEE, 2019.    0
    % \item He, Youbiao, Gihan J. Mendis, and Jin Wei. "Real-time detection of false data injection attacks in smart grid: A deep learning-based intelligent mechanism." IEEE Transactions on Smart Grid 8, no. 5 (2017): 2505-2516. not checked
    \item Nanduri, Anvardh, and Lance Sherry. "Anomaly detection in aircraft data using Recurrent Neural Networks (RNN)." In 2016 Integrated Communications Navigation and Surveillance (ICNS), pp. 5C2-1. IEEE, 2016. 68 c
    
\end{itemize}

Web of Science:
\begin{itemize}
    % \item Wang, Xiao, Quan Zhou, Jacob Harer, Gavin Brown, Shangran Qiu, Zhi Dou, John Wang, Alan Hinton, Carlos Aguayo Gonzalez, and Peter Chin. "Deep learning-based classification and anomaly detection of side-channel signals." In Cyber Sensing 2018, vol. 10630, p. 1063006. International Society for Optics and Photonics, 2018.      7 not cps
    \item Wang, Huaizhi, Jiaqi Ruan, Zhengwei Ma, Bin Zhou, Xueqian Fu, and Guangzhong Cao. "Deep learning aided interval state prediction for improving cyber security in energy internet." Energy 174 (2019): 1292-1304. 2 c
    % \item Muna, AL-Hawawreh, Nour Moustafa, and Elena Sitnikova "Identification of malicious activities in industrial internet of things based on deep learning models." Journal of Information Security and Applications 41 (2018): 1-11.  2   not cps data
    % \item Araya, Daniel B., Katarina Grolinger, Hany F. ElYamany, Miriam AM Capretz, and Girma Bitsuamlak. "An ensemble learning framework for anomaly detection in building energy consumption." Energy and Buildings 144 (2017): 191-206.  44 not clear
    \item Wu, Zhenyu, Yang Guo, Wenfang Lin, Shuyang Yu, and Yang Ji. "A weighted deep representation learning model for imbalanced fault diagnosis in cyber-physical systems." Sensors 18, no. 4 (2018): 1096.       8  c
    % \item Kang, Min-Joo, and Je-Won Kang. "Intrusion detection system using deep neural network for in-vehicle network security." PloS one 11, no. 6 (2016): e0155781. not checked  not good
\end{itemize}


Science direct:
\begin{itemize}
    \item Basumallik, Sagnik, Rui Ma, and Sara Eftekharnejad. "Packet-data anomaly detection in PMU-based state estimator using convolutional neural network." International Journal of Electrical Power \& Energy Systems 107 (2019): 690-702.      3  c
    % \item Huang, Tian-en, Qinglai Guo, Hongbin Sun, Chin-Woo Tan, and Tianyu Hu. "A deep spatial-temporal data-driven approach considering microclimates for power system security assessment." Applied energy 237 (2019): 36-48.  2 not cps
    \item   Li, Zhe, Jingyue Li, Yi Wang, and Kesheng Wang. "A deep learning approach for anomaly detection based on SAE and LSTM in mechanical equipment." The International Journal of Advanced Manufacturing Technology (2019): 1-12.    0     c
    % \item Bae, Gimin, Sunggyun Jang, Minseop Kim, and Inwhee Joe. "Autoencoder-Based on Anomaly Detection with Intrusion Scoring for Smart Factory Environments." In International Conference on Parallel and Distributed Computing: Applications and Technologies, pp. 414-423. Springer, Singapore, 2018.     0 junk
    \item Fan, Cheng, Fu Xiao, Yang Zhao, and Jiayuan Wang. "Analytical investigation of autoencoder-based methods for unsupervised anomaly detection in building energy data." Applied energy 211 (2018): 1123-1135.  24 c
    \item Lindemann, Benjamin, Fabian Fesenmayr, Nasser Jazdi, and Michael  Weyrich. "Anomaly detection in discrete manufacturing using self-learning approaches." Procedia CIRP 79 (2019): 313-318.  0  c
    \item Habler, Edan, and Asaf Shabtai. "Using LSTM encoder-decoder algorithm for detecting anomalous ADS-B messages." Computers \& Security 78 (2018): 155-173.  7 c  
    % \item Fengming, Zheng, Li Shufang, Guo Zhimin, Wu Bo, Tian Shiming, and Pan Mingming. "Anomaly detection in smart grid based on encoder-decoder framework with recurrent neural network." The Journal of China Universities of Posts and Telecommunications 24, no. 6 (2017): 67-73.  4 too low
    \item Canizo, Mikel, Isaac Triguero, Angel Conde, and Enrique Onieva. "Multi-head CNN–RNN for multi-time series anomaly detection: An industrial case study." Neurocomputing (2019). 0 c
 
\end{itemize}


survey
\begin{itemize}
    % \item Jiang, Dianbin, and Jingling Zhao. "Machine Learning in Industrial Control System Security: A Survey." In Chinese Intelligent Systems Conference, pp. 310-317. Springer, Singapore, 2019.
    \item Mohammadi, Mehdi, Ala Al-Fuqaha, Sameh Sorour, and Mohsen Guizani. "Deep learning for IoT big data and streaming analytics: A survey." IEEE Communications Surveys \& Tutorials 20, no. 4 (2018): 2923-2960.
    \item Hindy, Hanan, David Brosset, Ethan Bayne, Amar Seeam, Christos Tachtatzis, Robert Atkinson, and Xavier Bellekens. "A taxonomy and survey of intrusion detection system design techniques, network threats and datasets." arXiv preprint arXiv:1806.03517 (2018).    16
    \item Chandre, Pankaj R., Parikshit N. Mahalle, and Gitanjali R. Shinde. "Deep Learning and Machine Learning Techniques for Intrusion Detection and Prevention in Wireless Sensor Networks: Comparative Study and Performance Analysis." In Design Frameworks for Wireless Networks, pp. 95-120. Springer, Singapore, 2020.
    \item Diez-Olivan, Alberto, Javier Del Ser, Diego Galar, and Basilio Sierra. "Data fusion and machine learning for industrial prognosis: Trends and perspectives towards industry 4.0." Information Fusion 50 (2019): 92-111.   29
    \item Ratasich, Denise, Faiq Khalid, Florian Geissler, Radu Grosu, Muhammad Shafique, and Ezio Bartocci. "A roadmap toward the resilient internet of things for cyber-physical systems." IEEE Access 7 (2019): 13260-13283.      4
    \item Dekhtiar, Jonathan, Alexandre Durupt, Matthieu Bricogne, Benoit Eynard, Harvey Rowson, and Dimitris Kiritsis. "Deep learning for big data applications in CAD and PLM–Research review, opportunities and case study." Computers in Industry 100 (2018): 227-243.  5
    \item Zhao, Rui, Ruqiang Yan, Zhenghua Chen, Kezhi Mao, Peng Wang, and Robert X. Gao. "Deep learning and its applications to machine health monitoring." Mechanical Systems and Signal Processing 115 (2019): 213-237.
    \item Khan, Samir, Chun Fui Liew, Takehisa Yairi, and Richard McWilliam. "Unsupervised anomaly detection in unmanned aerial vehicles." Applied Soft Computing 83 (2019): 105650.
    \item Wang, Hongzhi, Mohamed Jaward Bah, and Mohamed Hammad. "Progress in Outlier Detection Techniques: A Survey." IEEE Access 7 (2019): 107964-108000.
    \item Loukas, George, Eirini Karapistoli, Emmanouil Panaousis, Panagiotis Sarigiannidis, Anatolij Bezemskij, and Tuan Vuong. "A taxonomy and survey of cyber-physical intrusion detection approaches for vehicles." Ad Hoc Networks 84 (2019): 124-147.
    \item Wu, Wufei, Renfa Li, Guoqi Xie, Jiyao An, Yang Bai, Jia Zhou, and Keqin Li. "A Survey of Intrusion Detection for In-Vehicle Networks." IEEE Transactions on Intelligent Transportation Systems (2019).
    \item Wickramasinghe, Chathurika S., Daniel L. Marino, Kasun Amarasinghe, and Milos Manic. "Generalization of Deep Learning for Cyber-Physical System Security: A Survey." In IECON 2018-44th Annual Conference of the IEEE Industrial Electronics Society, pp. 745-751. IEEE, 2018. not much useful info
    % \item Valliammal, N., and Barani Shaju. "Deep learning algorithm based cyber-attack detection in cyber-physical systems-a survey." International Journal of Advanced Technology and Engineering Exploration 5, no. 49 (2018): 489-494. related junk
    
\end{itemize}


springer
\begin{itemize}
    % \item García, Joel, Erik Zamora, and Humberto Sossa. "Supervised and unsupervised neural networks: Experimental study for anomaly detection in electrical consumption." In Mexican International Conference on Artificial Intelligence, pp. 98-109. Springer, Cham, 2018. 1 junk paper
    \item Ezeme, Okwudili M., Michael Lescisin, Qusay H. Mahmoud, and Akramul Azim. "DeepAnom: An Ensemble Deep Framework for Anomaly Detection in System Processes." In Canadian Conference on Artificial Intelligence, pp. 549-555. Springer, Cham, 2019. 0  c
    \item Khan, Haider Adnan, Nader Sehatbakhsh, Luong N. Nguyen, Milos Prvulovic, and Alenka Zajić. "Malware Detection in Embedded Systems Using Neural Network Model for Electromagnetic Side-Channel Signals." Journal of Hardware and Systems Security (2019): 1-14. 0 c
    % \item Naeem, Hamad. "Detection of Malicious Activities in Internet of Things Environment Based on Binary Visualization and Machine Intelligence." Wireless Personal Communications (2019): 1-21.  1 not anomaly detection
    \item Xiao, Yu-jun, Wen-yuan Xu, Zhen-hua Jia, Zhuo-ran Ma, and Dong-lian Qi. "NIPAD: a non-invasive power-based anomaly detection scheme for programmable logic controllers." Frontiers of Information Technology \& Electronic Engineering 18, no. 4 (2017): 519-534. 6  c
    % \item Rettig, Oliver, Silvan Müller, Marcus Strand, and Darko Katic. "Which deep artifical neural network architecture to use for anomaly detection in Mobile Robots kinematic data?." In Machine Learning for Cyber Physical Systems, pp. 58-65. Springer Vieweg, Berlin, Heidelberg, 2019. 0 not real anomaly detection
    % \item Kalinin, Maxim O., Daria S. Lavrova, and A. V. Yarmak. "Detection of Threats in Cyberphysical Systems Based on Deep Learning Methods Using Multidimensional Time Series." Automatic Control and Computer Sciences 52, no. 8 (2018): 912-917. 5 junk
    % \item Karray, Khaled, Jean-Luc Danger, Sylvain Guilley, and Moulay Abdelaziz Elaabid. "Prediction-Based Intrusion Detection System for In-Vehicle Networks Using Supervised Learning and Outlier-Detection." In IFIP International Conference on Information Security Theory and Practice, pp. 109-128. Springer, Cham, 2018. 0 not deep learning
    % \item Lokman, Siti Farhana, Abu Talib Othman, Shahrulniza Musa, and Muhamad Husaini Abu Bakar. "Deep Contractive Autoencoder-Based Anomaly Detection for In-Vehicle Controller Area Network (CAN)." In Progress in Engineering Technology, pp. 195-205. Springer, Cham, 2019. 0 junk
    \item Jichici, Camil, Bogdan Groza, and Pal-Stefan Murvay. "Examining the Use of Neural Networks for Intrusion Detection in Controller Area Networks." In International Conference on Security for Information Technology and Communications, pp. 109-125. Springer, Cham, 2018. 0  c
    % \item Nabil, Mahmoud, Muhammad Ismail, Mohamed Mahmoud, Mostafa Shahin, Khalid Qaraqe, and Erchin Serpedin. "Deep Learning-Based Detection of Electricity Theft Cyber-Attacks in Smart Grid AMI Networks." In Deep Learning Applications for Cyber Security, pp. 73-102. Springer, Cham, 2019. 0 not cps feature
    \item Wang, Yawei, Donghui Chen, Cheng Zhang, Xi Chen, Baogui Huang, and Xiuzhen Cheng. "Wide and Recurrent Neural Networks for Detection of False Data Injection in Smart Grids." In International Conference on Wireless Algorithms, Systems, and Applications, pp. 335-345. Springer, Cham, 2019. 0 c
    \item Li, Dan, Dacheng Chen, Baihong Jin, Lei Shi, Jonathan Goh, and See-Kiong Ng. "MAD-GAN: Multivariate anomaly detection for time series data with generative adversarial networks." In International Conference on Artificial Neural Networks, pp. 703-716. Springer, Cham, 2019. 8 c
\end{itemize}


open
\begin{itemize}
    % \item  Unsupervised Learning for Online Abnormality Detection in Smart Meter Data
    \item Long Short Term Memory Networks for
Anomaly Detection in Time Series 331   not complete
    \item Liu, Chao, Kin Gwn Lore, Zhanhong Jiang, and Soumik Sarkar. "Root-cause Analysis for Time-series Anomalies via Spatiotemporal Graphical Modeling in Distributed Complex Systems." arXiv preprint arXiv:1805.12296 (2018).  1
    \item Zhou, Aiguo, Zhenyu Li, and Yong Shen. "Anomaly Detection of CAN Bus Messages Using A Deep Neural Network for Autonomous Vehicles." Applied Sciences 9, no. 15 (2019): 3174.   0
    \item Yang, Yanqing, Kangfeng Zheng, Chunhua Wu, and Yixian Yang. "Improving the Classification Effectiveness of Intrusion Detection by Using Improved Conditional Variational AutoEncoder and Deep Neural Network." Sensors 19, no. 11 (2019): 2528.    0
    \item Sadhu, Vidyasagar, Teruhisa Misu, and Dario Pompili. "Deep Multi-Task Learning for Anomalous Driving Detection Using CAN Bus Scalar Sensor Data." arXiv preprint arXiv:1907.00749 (2019).   0
    \item Burak Gunay, H., Weiming Shen, Guy Newsham, and Araz Ashouri. "Detection and interpretation of anomalies in building energy use through inverse modeling." Science and Technology for the Built Environment 25, no. 4 (2019): 488-503.   0
    \item Malhotra, Pankaj, Anusha Ramakrishnan, Gaurangi Anand, Lovekesh Vig, Puneet Agarwal, and Gautam Shroff. "LSTM-based encoder-decoder for multi-sensor anomaly detection." arXiv preprint arXiv:1607.00148 (2016).  117
    \item He, Zecheng, Aswin Raghavan, Sek Chai, and Ruby Lee. "Detecting zero-day controller hijacking attacks on the power-grid with enhanced deep learning." arXiv preprint arXiv:1806.06496 (2018).   3
    \item Eiteneuer, Benedikt, and Oliver Niggemann. "LSTM for Model-based Anomaly Detection in Cyber-Physical Systems." In DX@ Safeprocess. 2018. 
    \item Meng, Hengyu, Yuxuan Zhang, Yuanxiang Li, and Honeghua Zhao. "Spacecraft anomaly detection via transformer reconstruction error."  0
    \item Malhotra, Pankaj, Vishnu TV, Anusha Ramakrishnan, Gaurangi Anand, Lovekesh Vig, Puneet Agarwal, and Gautam Shroff. "Multi-sensor prognostics using an unsupervised health index based on lstm encoder-decoder." arXiv preprint arXiv:1608.06154 (2016). 48
    \item Guo, Yifan, Weixian Liao, Qianlong Wang, Lixing Yu, Tianxi Ji, and Pan Li. "Multidimensional time series anomaly detection: A gru-based gaussian mixture variational autoencoder approach." In Asian Conference on Machine Learning, pp. 97-112. 2018.   4
    \item DyAt Nets: Dynamic Attention Networks for State Forecasting
in Cyber-Physical Systems 0
    \item He, Miao. "Development of Deep Learning Based Methodology on Rotating Machine Fault Diagnosis." PhD diss., 2018. 
    \item Kravchik, Moshe, and Asaf Shabtai. "Efficient Cyber Attacks Detection in Industrial Control Systems Using Lightweight Neural Networks." arXiv preprint arXiv:1907.01216 (2019).   0
    \item Akerman, Sefi, Edan Habler, and Asaf Shabtai. "VizADS-B: Analyzing Sequences of ADS-B Images Using Explainable Convolutional LSTM Encoder-Decoder to Detect Cyber Attacks." arXiv preprint arXiv:1906.07921 (2019). 1
    \item Lokman, Siti Farhana, Abu Talib Othman, Muhamad Husaini Abu Bakar, and Rizal Razuwan. "Stacked sparse autoencoders-based outlier discovery for in-vehicle controller area network (CAN)." International Journal of Engineering \& Technology 7, no. 4.33 (2018): 375-380.   1
    \item Hanselmann, Markus, Thilo Strauss, Katharina Dormann, and Holger Ulmer. "CANet: An Unsupervised Intrusion Detection System for High Dimensional CAN Bus Data." arXiv preprint arXiv:1906.02492 (2019). 0
    \item Jiang, Wenqian, Cheng Cheng, Beitong Zhou, Guijun Ma, and Ye Yuan. "A Novel GAN-based Fault Diagnosis Approach for Imbalanced Industrial Time Series." arXiv preprint arXiv:1904.00575 (2019). 0
    \item Shalyga, Dmitry, Pavel Filonov, and Andrey Lavrentyev. "Anomaly Detection for Water Treatment System based on Neural Network with Automatic Architecture Optimization." arXiv preprint arXiv:1807.07282 (2018). 2
    \item Hasan, Md, Rafia Nishat Toma, Abdullah-Al Nahid, M. M. Islam, and Jong-Myon Kim. "Electricity Theft Detection in Smart Grid Systems: A CNN-LSTM Based Approach." Energies 12, no. 17 (2019): 3310. 0ICSicsICSICS
\end{itemize}

% ACM ML for AD in CPS:

% \begin{itemize}
%     \item Kreimel, Philipp, Oliver Eigner, and Paul Tavolato. "Anomaly-Based Detection and Classification of Attacks in Cyber-Physical Systems." In Proceedings of the 12th International Conference on Availability, Reliability and Security, p. 40. ACM, 2017.

%TABOR: A Graphical Model-based Approach for Anomaly Detection in Industrial Control Systems

%Behaviour-Based Attack Detection and Classification in Cyber Physical Systems Using Machine Learning

% \end{itemize}

==> sections/cases.tex <==
\section{Public datasets}
DLAD methods usually require a large volume of data to train and test neural models. It is important and essential to collect datasets for DLAD methods. In this section, we present publicly available datasets used in existing work. We summarize the characteristics of these datasets from (1) Systems and devices. The specific systems and devices where data is collected. (2) Period. When and how long the data has been collected. (3) Data types and size. Data types include sensors, actuators, network traffic, control system logs and commands, time series. (4) Attack or fault. We report the characteristics of attack or fault cases (if any). We list all available datasets in Table~\ref{datasettable}.



\subsection{\textsc{Datasets used in ICSs}}
\textit{SWaT}. SWaT~\cite{itrust} is a six-stage scale-down water treatment testbed for research purposes, which implements main functionalities in a real-world water treatment plant. The raw water is pumped into the testbed at the first stage. The following four stages utilize chemical and physical processes (\eg, Ultrafiltration (UF) and Reverse Osmosis (RO) systems) to filter and generate pure water. The final stage is a backwash step to the UF system. The physical devices include pumps, sensors (\eg, the level of water, flow speed), tanks, and chemical/physical treatment devices. The cyber systems consist of a communication network, programmable logic controllers (PLCs) and the SCADA system. The dataset collected 7 days of normal data and 4 days of attack cases. The sensor and actuator values are in time-series form and sampled one data point every second, which is 125MB in normal period and 111MB in the attack period. The dataset also provides 50 network traces of normal period (300GB) and two network traces of attack period (104GB).   36 attacks (\eg, false control signals, false sensor readings) are designed to simulate real-world attacks. At Aug. 2019, the dataset updated with three hours of normal and one hour of attack data.

\textit{Modbus network data}. Modbus is one of the communication protocols used in SCADA systems. Lemay \etal~\cite{lemay2016providing} developed a SCADA sandbox to generate normal and attack Modbus network traffic. The sandbox consists of Master Terminal Units (MTUs), controllers and field devices. For each simulated case, the traffic capturing duration varies from 1 minute to 1 hour. The dataset provides 6 normal and 5 attack network traces, which is configured under different MTU and Remote Terminal Unit (RTU) settings. The size of each trace ranges from 1426 to 305932 entries. The attacks include malware and false control signals. The dataset can be downloaded at \cite{modbus_dataset_2019}.

\textit{Tennessee Eastman process (TEP) simulation}. TEP simulates a realistic setting of a chemical plant, which consists of a reactor, condenser, compressor, separator, and stripper. Totally, 53 measurements are collected from the system, of which 41 are normal values while 12 are manipulated. The normal measurements include temperature, level, pressure, flow, \etc. The anomalous readings are feed flow, purge valve, steam valve, cooling water flow, \etc. Since this simulation framework has been used in multiple methods~\cite{liu2017data, russell2012data, yin2012comparison, chiang2000fault}, we adopt a well-documented version presented in \cite{rieth2017additional}. The dataset includes the fault-free train (23MB), fault-free test (45MB), fault train (471MB), and fault test (798MB) versions of data. The training and testing datasets run for 25 and 48 hours respectively, which are sampled every 3 minutes. Specifically, twenty-one faults are designed to create anomalies in the system, which includes fixed sensor readings, random variation and the slow drift of sensor values, \etc. The dataset is available at \cite{rieth_additional_2017}. The simulator can be obtained at \cite{tepcode}.

\input{sections/datasettable.tex}

\textit{Gas pipeline testbed}. Morris \etal~\cite{morris2015industrial} built a laboratory-scale gas pipeline system, where Modbus network traffic data in the SCADA system was generated. The testbed consists of a pump, valve, pipeline, fluid flow, and air compressor. A proportional integral derivative (PID) controller is adopted to manage air pressure. Twenty features are captured from traffic data in the dataset, \ie, the length of the packet, the pressure setpoint, PID related information, pressure, \etc. The dataset is 17MB and contains 214580 normal traffic packets and 60048 packets in the attack period. There are three categories of attacks, \eg, packet injection, DoS, MITM. The dataset is available at \cite{ndustrial_pipeline}.

\textit{Smart Home Technology (REFIT) dataset}. REFIT is a research project that studies buildings, users, energy, communication, and design in UK homes~\cite{refit}. The project carried out surveys and interviews to understand the perceptions of smart homes and qualitative data on electricity and gas usage. Also, measurement data is collected in real-world households from field sensors and devices. Four datasets focus on different aspects of smart homes in the REFIT project. We report the REFIT smart home dataset~\cite{refit_2017} that is used in one DLAD method~\cite{legrand2018study}. The devices include thermostats, valves, meters and motion, door, window sensors in 20 homes. The data was collected from October 2014 to April 2015. A description of the location, construction details, energy services of homes is provided. Then, power load, gas usage, temperature, user activity sensors are monitored to form the time-series dataset, which is 94MB. There is no attack or fault in the dataset. 

\textit{PHM 2015 Challenge}. This challenge provides the running status of real industrial plants, which includes time-series sensor measurements, control signals data, and fault events. The devices mainly comprise Heating, ventilation, and air conditioning (HAVC) and some electricity meters. The data sampling frequency is 15 minutes and the collection lasts around three years, which ranges from 2010 to 2012. For each HAVC, sensors 1 to 4  (no details) and control status 1 to 4 are recorded. Meanwhile, the instant power and electricity consumption of each zone are reported. Totally, the dataset contains 70 plants, whose size is about 390MB. Five types of faults are produced in each plant, which covers abnormal temperature, wrong temperature setpoint, wrong cooling zone, \etc. The dataset is available at \cite{phm}.



\subsection{\textsc{Datasets used in smart grid}}
\textit{New York Independent System Operator (NYISO)}. NYISO is responsible for managing the power grid and marketplace in New York, while it does not operate or own the infrastructure. It publishes the market and operational data (\ie, pricing, power grid transmission, load data) every day. The load data is used by one work~\cite{deng2018false} to simulate a more real power grid. Researchers could also get pricing and transmission data. The dataset begins in May 2001 and keeps updating daily. Power load data of 11 areas in New York are recorded every five seconds, whose size is about 160KB each day. There is no attack or fault data in the dataset. The dataset is available at \cite{NYISO_load}.

\textit{IEEE X-bus system}. IEEE X-bus test system~\cite{buayai2014applied, ieee_bus_electric} is an approximation of the American Electric Power system, which is developed to simulate the power grid system in the U.S. Depending on the bus quantity and network topologies, there are 14, 24, 30, 39, 57, 118-bus systems. The devices include buses, generators, transformers, synchronous condensers, lines. Since it is a simulation platform, researchers can collect simulated data for any period. Voltage, current, and frequency measurements can be recorded in the system. Typically, data from a real power grid can be loaded into the system to generate more realistic scenarios. Though the system does not provide attack or fault cases, users can inject manually created attacks and faults (\eg, FDI) to simulate anomalies. 

\subsection{\textsc{Datasets used in ITSs}}
\textit{Safety Pilot Model Deployment (SPMD) program}.  The SPMD program is to advance vehicle-to-vehicle (V2V) and vehicle-to-infrastructure (V2I) communications with a real environment, equipment, and deployment, which is performed by the University of Michigan. Vehicle awareness devices (VADs) and aftermarket safety devices (ASDs) are installed on over 2500 real passenger vehicles to support safety-ensuring communication messages. From August 2012 to February 2014, the V2V data was collected. Brake events, basic safety messages (BSM), front targets, GPS, radar and network traffic statistics information are published. The sensor data is about 3.2GB (\eg, brake, GPS, radar) and the network traffic is about 16GB (\eg, BSM). There are no attack or fault cases in the dataset. The description of the program is at \cite{smpd_teamreport} and the dataset is available at \cite{spmd_safety}. 

\textit{UAH-DriveSet driver behaviour data}. UAH-DriveSet utilizes six different types of passenger vehicles and six different drivers to perform driving behaviors on motorway and secondary road. Three driving strategies (\ie, normal way, drowsy or aggressive mode) are adopted. Real vehicles with multiple sensors are applied to capture data, which are used in the Naturalistic Driving Study~\cite{bender2016flexible}. Over 500 minutes of driving performance data are collected in 36 tests. Speed, altitude, acceleration, latitude, and longitude coordinate information are stored in the dataset, which is 3.3GB. Aggressive driving behaviors are considered anomalies, which will cause sensor measurements to be different from the normal driving period. The description is at \cite{romera2016need} while the dataset can be downloaded at \cite{uah-driveset}.

\textit{CAN Dataset for intrusion detection (OTIDS)}. OTIDS provides CAN bus traffic that is generated during in-vehicle communication between different nodes. The attack-free dataset includes 2.3 million messages. DoS attack (656K messages), fuzzy attack (591K messages), impersonation attack (1.6 million messages) messages are injected in a real vehicle. The description is at \cite{lee2017otids} and the dataset can be downloaded at \cite{can-intrusion-dataset}.

\subsection{\textsc{Datasets used in aerial systems}}
\textit{Soil Moisture Active Passive (SMAP) satellite}. SMAP is a satellite developed to monitor the soil moisture and freeze on Earth. The telemetry data between the satellite and control center is published by \cite{hundman2018detecting}. Time information is anonymized and data is scaled between -1 and 1. There are 55 telemetry channels in the dataset and each channel represents one aspect of a spacecraft, \eg, power. For each channel, there can be multiple sensors to measure the status. Totally, the dataset is 86MB. 43 point anomalies and 26 contextual anomalies are also given in the dataset, but the details are not presented. The dataset is available at \cite{hundman_khundmantelemanom_2020}.

\textit{Mars Science Laboratory (MSL) rover, Curiosity}. The curiosity's mission is to investigate whether there is evidence on Mars that the environment is habitable for humans. Telemetry data is transmitted to send control commands and receive measurement data. In the work~\cite{hundman2018detecting}, this data is published along with the SMAP project. The data is also scaled to (-1,1) and time values are deleted, where 27 telemetry channels are recorded. A telemetry stream consists of several control commands and a telemetry value. Also, 19 point anomalies and 17 contextual anomalies are used as anomalous data. The details of the anomalies are not shown in the paper. Researchers can download the dataset at \cite{hundman_khundmantelemanom_2020}.

\textit{Logs from a UAV platform}. This dataset offers kernel event logs from QNX RTOS operating system traces on a UAV platform. The UAV is operated in four modes, which are full-while, fifo-ls, hilRF-InFin, and sporadic. Each scenario contains training samples, validation cases, and anomalies. Multiple traces of a scenario are generated when experimenting, each of which contains 50000 samples. Four types of attacks are introduced. The first attack runs a loop to exhaust CPU computing resources. The other two attacks schedule interfering tasks to interrupt normal operations. The last attack runs in a normal mode but deviates from training samples. The description of the dataset is at \cite{salem2016anomaly}.

\textit{Flightradar24}. ADS-B messages, which are used by aircraft to broadcast position and running status information,  are utilized in the work~\cite{habler2018using} to build an LSTM-based anomaly detection method. Aircraft identification, position, velocities, status information can be contained in the message. In the work~\cite{habler2018using}, over 800 flights from 14 airports are adopted, which range from March 2017 to April 2018. No anomaly cases are in the dataset, while the authors manually injected abnormal messages. ADS-B messages can be accessed at Flightradar24~\cite{flightradar24}. 

% \subsection{Cases}

% \begin{itemize}
%     \item multiple serious security flaws in the code for a component of the 787 known as a Crew Information Service/Maintenance System, blackhat 2019
%     \item Ukraine power plant
%     \item the Stuxnet worm
% \end{itemize}



==> sections/curentDLmethodstable.tex <==


















\begin{table}[h]
\centering
\caption{Deep learning-based anomaly detection methods in ICS}
\Large

\resizebox{12cm}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
paper                                                                                                                                                & Model                                                              & \begin{tabular}[c]{@{}l@{}}Anomaly\\ score\end{tabular}                                 & \begin{tabular}[c]{@{}l@{}}Source\\ Code\end{tabular} & Data                                                   & \begin{tabular}[c]{@{}l@{}}Data \\ type\end{tabular}                      & Time \\ \hline
\begin{tabular}[c]{@{}l@{}}A Deep Neural Network for Unsupervised \\ Anomaly Detection and Diagnosis in\\ Multivariate Time Series Data\end{tabular} & \begin{tabular}[c]{@{}l@{}}CNN+ConvLSTM\\ Autoencoder\end{tabular} & \begin{tabular}[c]{@{}l@{}}reconstruction\\ error\end{tabular}                          & \begin{tabular}[c]{@{}l@{}}not\\ public\end{tabular}  & \begin{tabular}[c]{@{}l@{}}not\\ public\end{tabular}   & \begin{tabular}[c]{@{}l@{}}sensor\\ time\\ series\end{tabular}            & 2019 \\ \hline
\begin{tabular}[c]{@{}l@{}}MAD-GAN: Multivariate Anomaly Detection for Time\\ Series Data with Generative Adversarial Networks\end{tabular}          & GAN                                                                & \begin{tabular}[c]{@{}l@{}}reconstruction\\ error\\ discrimination\\ error\end{tabular} & public                                                & \begin{tabular}[c]{@{}l@{}}SWaT\\ WADI\end{tabular}    & \begin{tabular}[c]{@{}l@{}}sensor\&\\ actuator\\ time series\end{tabular} & 2019 \\ \hline
\begin{tabular}[c]{@{}l@{}}Detecting Cyber Attacks in Industrial Control \\ Systems Using Convolutional Neural Networks\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}1D CNN+\\ LSTM\end{tabular}             & prediction error                                                                        & \begin{tabular}[c]{@{}l@{}}not\\ public\end{tabular}  & SWaT                                                   & \begin{tabular}[c]{@{}l@{}}sensor\&actuator\\ time series\end{tabular}    & 2018 \\ \hline
\begin{tabular}[c]{@{}l@{}}Efficient Cyber Attacks Detection in Industrial Control \\ Systems Using Lightweight,Neural Networks\end{tabular}         & \begin{tabular}[c]{@{}l@{}}1D CNN+\\ Autoencoder\end{tabular}      & \begin{tabular}[c]{@{}l@{}}reconstruction\\ error\end{tabular}                          & \begin{tabular}[c]{@{}l@{}}not\\ public\end{tabular}  & \begin{tabular}[c]{@{}l@{}}SWaT\\ Batadal\end{tabular} & \begin{tabular}[c]{@{}l@{}}sensor\&actuator\\ time series\end{tabular}    & 2019 \\ \hline
\end{tabular}
}
\end{table}




==> sections/datasettable.tex <==
\begin{table}[]
\caption{Summary of publicly available datasets used in existing work. \enquote{\CIRCLE}, \enquote{-}, \enquote{\LEFTcircle} means \enquote{Yes}, \enquote{Does not apply}, and \enquote{Does not clear but inferred to be Yes} respectively. \enquote{D}, \enquote{H} means \enquote{Day} and \enquote{Hour}. \enquote{$\approx$} means \enquote{approximately}. }
\vspace{5pt}

\resizebox{14cm}{!}{
%\hspace{-1.5cm}
\begin{tabular}{c|c|c|c|cV{5}c|c|c|c|c|cV{5}c|c|c|c|cV{5}c|c|c}
\hline
\cellcolor{lightgray}{\textbf{Name} } & \cellcolor{lightgray}{\textbf{Domain} }     & \cellcolor{lightgray} {\textbf{Description}} & \cellcolor{lightgray}{\textbf{When}} & \cellcolor{lightgray}{\textbf{Period}} & \multicolumn{6}{cV{5}}{  \cellcolor{lightgray} {\textbf{Data type} }  }                                                        & \multicolumn{5}{cV{5}}{  \cellcolor{lightgray}{\textbf{Attacks} }  }                                     & \multicolumn{3}{c}{ \cellcolor{lightgray}{\textbf{Faults} }}                    \\ \hline
     &        &     &      &        &  \rot{\begin{tabular}[c]{@{}c@{}} \textbf{Sensor/Actuator} \\ \textbf{reading}\end{tabular}} & \rot{\textbf{Size}} & \rot{\textbf{Network traffic}} & \rot{\textbf{Size}} & \rot{\textbf{Control system logs}} & \rot{\textbf{Size}} & \rot{\textbf{DoS}} & \rot{\textbf{MITM}} & \rot{\textbf{Packet injection}} & \rot{\textbf{Malware}} & \rot{\textbf{False control signals}} & \rot{\textbf{Sensor layer}} & \rot{\textbf{Network layer}} & \rot{\textbf{Control system}}      \\ \hline \hline
SWaT\cite{itrust}      & ICS &  \begin{tabular}[c]{@{}c@{}}A scale-down water \\ treatment testbed\end{tabular}         &   2015   &   11D     &     \CIRCLE     &  236MB    & \CIRCLE    &   404GB   &     -    &   -   &  -   &   \CIRCLE     &    -              &    -     &     \CIRCLE     &  -   &   - &  -    \\ \hline

Modbus\cite{lemay2016providing} &  ICS &\begin{tabular}[c]{@{}c@{}} Simulated Modbus \\ network traffic data  \end{tabular}  & 2016 & $\approx7H$ & - & - &  \CIRCLE & \begin{tabular}[c]{@{}c@{}}  $\approx 912K $\\ entries  \end{tabular} & - & - & - & - & - &  \CIRCLE &  \CIRCLE & - & - & - \\ \hline
TEP\cite{rieth_additional_2017} &    ICS     &\begin{tabular}[c]{@{}c@{}} Simulated \\ chemical plant \end{tabular}  & 2017 & 146H & \CIRCLE & 1.3GB & - & - & - & - & - & - & - & - & - & \CIRCLE  & - & -  \\ \hline
\begin{tabular}[c]{@{}c@{}} Gas  pipeline\cite{morris2015industrial} \end{tabular} &   ICS      & \begin{tabular}[c]{@{}c@{}}  Gas pipeline \\testbed \end{tabular}  & 2015 & - & - & - &  \CIRCLE & 17MB & - & - &  \CIRCLE &  \CIRCLE &  \CIRCLE  & - & - & - & - & -   \\ \hline
\begin{tabular}[c]{@{}c@{}} REFIT  smart home\cite{refit_2017} \end{tabular}&    ICS     & \begin{tabular}[c]{@{}c@{}}  Smart home \\ measurements  \end{tabular} & 2015 & 7Months &  \CIRCLE  & 94MB & - & - & - & - & - & - & - & - & - & - & - & - \\ \hline

\begin{tabular}[c]{@{}c@{}} PHM 2015 Challenge\cite{phm} \end{tabular}&  ICS    & \begin{tabular}[c]{@{}c@{}}  Plant measurements  \end{tabular} & 2015 & 3Years &  \CIRCLE  & 390MB & - & - & - & - & - & - & - & - & - & \CIRCLE  & - & \CIRCLE  \\ \hline

\begin{tabular}[c]{@{}c@{}} NYISO\cite{NYISO_load}  \end{tabular} & \begin{tabular}[c]{@{}c@{}}  Smart \\ grid   \end{tabular}    & \begin{tabular}[c]{@{}c@{}}  Power grid pricing, \\transmission, load data  \end{tabular} & Present & 19Years & -  & - & - & - &  \CIRCLE &  \begin{tabular}[c]{@{}c@{}}160\\KB/day \end{tabular}& - & - & - & - & - & -  & - & -   \\ \hline

\begin{tabular}[c]{@{}c@{}} IEEE X-bus system \cite{buayai2014applied}  \end{tabular} &  \begin{tabular}[c]{@{}c@{}}  Smart \\ grid   \end{tabular}    & \begin{tabular}[c]{@{}c@{}}  Power grid simulation  \end{tabular} & - & - & \CIRCLE  & - & - & - &  - & - & - & - & - & - & - & -  & - & -   \\ \hline

\begin{tabular}[c]{@{}c@{}} SPMD \cite{smpd_teamreport}  \end{tabular} &   ITS  & \begin{tabular}[c]{@{}c@{}}  Safety pilot model \\deployment program  \end{tabular} & 2014 & 2Years & \CIRCLE & 3.2GB &  \CIRCLE & 16GB &  - & - & - & - & - & - & - & -  &  - & -  \\ \hline

\begin{tabular}[c]{@{}c@{}} UAH DriveSet\cite{romera2016need}  \end{tabular} &  ITS  & \begin{tabular}[c]{@{}c@{}}  Driver behaviour \\ data  \end{tabular} & 2016 & $ \approx8H $& \CIRCLE & 3.3GB &  - & - &  - & - & - & - & - & - & - & \CIRCLE  &  - & -   \\ \hline

\begin{tabular}[c]{@{}c@{}} OTIDS \cite{lee2017otids}  \end{tabular} &  ITS   & \begin{tabular}[c]{@{}c@{}}  CAN bus traffic   \end{tabular} & 2017 & \begin{tabular}[c]{@{}c@{}}   $ \approx42 $\\Minutes   \end{tabular}   & - & - &  \CIRCLE  & 392M &  - & - & \CIRCLE & \CIRCLE & \CIRCLE & - & - & -  &  - & -   \\ \hline

\begin{tabular}[c]{@{}c@{}} SMAP\cite{hundman_khundmantelemanom_2020}  \end{tabular} & \begin{tabular}[c]{@{}c@{}} Aerial \\ systems  \end{tabular}  & \begin{tabular}[c]{@{}c@{}}  Telemetry data \\of a satellite  \end{tabular} & - & - & -  & - &  \CIRCLE & 86MB &  - & - & - & - & - & - & - & -  &  \CIRCLE & \LEFTcircle   \\ \hline

\begin{tabular}[c]{@{}c@{}} Curiosity \cite{hundman_khundmantelemanom_2020} \end{tabular} & \begin{tabular}[c]{@{}c@{}} Aerial \\ systems  \end{tabular} & \begin{tabular}[c]{@{}c@{}}  Telemetry data \\of a rover  \end{tabular} & - & - & -  & - &  \CIRCLE & 86MB &  - & - & - & - & - & - & - & -  &  \CIRCLE & \LEFTcircle  \\ \hline

\begin{tabular}[c]{@{}c@{}} UAV kernel events\cite{salem2016anomaly} \end{tabular} & \begin{tabular}[c]{@{}c@{}} Aerial \\ systems  \end{tabular} & \begin{tabular}[c]{@{}c@{}}  Kernel event traces \\ of a UAV  \end{tabular} & 2016 & - & -  & - &  - & - &  \CIRCLE  & - & \CIRCLE  & - & - & \CIRCLE & - & -  & - & - \\ \hline

\begin{tabular}[c]{@{}c@{}} Flightradar24\cite{flightradar24} \end{tabular}& \begin{tabular}[c]{@{}c@{}} Aerial \\ systems  \end{tabular}  & \begin{tabular}[c]{@{}c@{}}  ADS-B messages  \end{tabular} & - & - & -  & - &  \CIRCLE  & - &  -  & - & - & - & - & - & - & -  & - & -  \\ \hline


\end{tabular}
}
\label{datasettable}
\end{table}
